An Exploratory Study of Field Failures

Field failures, that is, failures caused by faults that escape the testing phase leading to failures in the field, are unavoidable. Improving verification and validation activities before deployment can identify and timely remove many but not all faults, and users may still experience a number of annoying problems while using their software systems. This paper investigates the nature of field failures, to understand to what extent further improving in-house verification and validation activities can reduce the number of failures in the field, and frames the need of new approaches that operate in the field. We report the results of the analysis of the bug reports of five applications belonging to three different ecosystems, propose a taxonomy of field failures, and discuss the reasons why failures belonging to the identified classes cannot be detected at design time but shall be addressed at runtime. We observe that many faults (70%) are intrinsically hard to detect at design-time.

==> opportunities.tex <==
\section{Test Obligations}

%The section might be structured as follows
%Test Obligations: (adequacy criterion), (give a name to each)
%what kind of coverage do we want (is not a real coverage, since it might be not bounded, but we are interested in increasing it),
%e.g. resources + functionality that use resources
%%better: all resources locations
%
%Failure trigger:
%resurce state, 
%e.g. location has changed, access not possible
%
%Failure scenario:
%generic ways to reach a state
%e.g. moving a resource
%e.g. renaming a resource
%
%Matching Failures:
%
%Test opportunity:
%check to be done at runtime to enable tests
%e.g. a resource has just been moved
%
%
%Oracle:
%Domain specific
%
%We may have multiple patterns for a same concrete fault
%
%TO: resource type
%FS: creating a resource of a specific subtype, e.g. new project with svn nature
%TO: new resource created
%

test obligations specify the general requirements of an application's testing process, specifically in this section we identify test obligations that are interesting in a field testing context. We associate multiple test opportunities to each obligation to identify and exploit potential testing situations that arise during the applications' regular use.

The test opportunities that we identify for each test obligation are derived from common \FFs{} patterns that emerge from the analysed data. Test opportunities exploit the obtained knowledge to determine how and when to execute tests during applications' regular use. 

\subsection{Obligation: functionality/resource coverage}

This obligation involves covering functionalities of our application after a resource used by such functionalities is modified or a new resource is introduced. A resource modification happens when the resource type, value, location or permissions change. More in detail we can specify the meaning of change for each of these categories:

\begin{itemize}
\item \emph{location}: a resource is deleted or moved to a different file system folder (local) or to a different URL (remote)
\item \emph{type}: resource format is modified
\item \emph{value}: resource contents are modified
\item \emph{permissions}: resource read/write permissions are modified
\end{itemize} 

\subsubsection{Pattern: modified resources location}

This pattern presents when a resource used by the application under test is no longer available at its original location. In general we have a specific resource $r$ in a location $l$ (with $L = \{l_1, l_2, ... l_n\}$ acceptable locations) used by some functionalities $F_r = \{f_1,f_2,...,f_n\}$. If $r$ is moved to a location $l'$ outside our set $L$ of acceptable locations, this might precede a failure in our application when the functionalities in $F_r$ try to manage the resource location change. \luca{why distinguish between abstract and concrete locations?}.

\paragraph{\textbf{Scenario}}
\smallskip
This scenario identifies situations where a failure is preceded by a relocation or deletion of resources used by the faulty functionality that triggers the failure. This happens when an external application or from a functionality other than the faulty one modifies a resource's location. The failure is typically triggered when the resource's location modification is handled by the faulty functionality. This scenario also allows us to define a rollback recovery strategy if the resources' location modification is done by a specific functionality inside our application.

\paragraph{\textbf{Matching failures}}

\paragraph{Subversive bug report 482565}
\smallskip
This is a Subversive fault which triggers a failure that manifests this way: the repository of an eclipse team multi-project is relocated, as soon as Eclipse starts it realizes that the relocation took place and it asks the user what to do; the user selects "Change repository location URL and relocate rest of projects" but after "ok" is hit when asked to relocate the first project the same prompt is shown in a loop. If "cancel" is hit after the loop starts the prompt for the relocation of the second project is shown, together with error reports.

\paragraph{Subversive bug report 373125}
\smallskip
This fault triggers a java.lang.IllegalArgumentException: Element not found exception when refactoring a project by moving its location from the Eclipse workspace to elsewhere in the file system. The failure is triggered because the refresh operation after the refactoring is split into several asynchronous parts.

\paragraph{Subversive bug report 480521}
\smallskip
To trigger the failure caused by this fault one may proceed in this way: move a Java class in an svn project to a different package and synchronize, then in Eclipse try to resolve conflicts; at this point an unhandled event loop exception is triggered.

\paragraph{EGit bug report 479964}
\smallskip
\luca{this fault is a bit borderline, it is not actually caused by relocation or deletion of resources but rather it handles deletion of resources in a wrong way, also it is categorized as "bad testing process"}

This fault triggers a failure when deleting an Eclipse project from the workspace if one selects and deselects the option "Also delete working tree". The failure is caused by the fact that the option "Remove the project in the repository from workspace" remains checked and hence the procedure deletes all contents on disk.

\paragraph{EGit bug report 413887}
\smallskip
\luca{this fault is a bit borderline, it is not actually caused by relocation or deletion of resources but when a new branch is created in the repository via EGit or when the repository is removed the system fails with an exception if non local project are present in the workspace (method IResource.getLocation() returns null) }


\paragraph{\textbf{Test Opportunity}}


\paragraph{Test Trigger}
\smallskip
We can simply take a resource location change from $l \in L$ to $l' \notin L$ as the trigger for the tests we defined. If the modification is performed by a functionality inside our testing set we can ignore the test cases that work on that functionality (the resource modification must come from another source).


\paragraph{Test Strategy}
\smallskip
It is clear that this failure pattern requires an application to use \emph{shared external resources} (repositories, files or databases for example), given this premise we can identify a test strategy that involves checking whether the shared resources have been relocated and that the functionalities that use them still work. To do this we need to monitor the current local and remote resources which the application can read/write and the list of the application's functionalities that perform these read/write operations (or the subset of them that we want to test). Once we have these elements we can test the functionalities that we selected when a modification on a shared resource is detected. In general we have a set of test suites $T = \{t_1,t_2,...,t_n\}$ in which each test suite tests a functionality, a set of resources $R = \{r_1, r_2,...,r_m\}$ and for each resource $r_i$ a set of allowed locations $L_i = \{l_{i1},l_{i2},...,l_{ik}\}$. We the identify $m$ subsets of $T$, $T_r = \{T_1,T_2,...,T_j\}$ where $T_i$ is the subset of test suites for the functionalities that use the $i^{th}$ resource in our list. When a resource $r_i$ inside $R$ is moved to a location $l'$ outside the set of allowed locations $L_i$ we execute all of the test suites in $T_i$.

\subsubsection{Pattern: new resources type}
%distingui a livello di strategia di test:
%risorsa esterna modificata solo dall'applicazione
%risorsa modificata dall'utente all'interno dell'applicazione
%input utente

This pattern requires some functionalities in the application under test to work on resources of different type. In this case the operations that the functionality applies to one type of resource might not work correctly on another type. The pattern presents when a functionality in the application that is usually applied to a resource of a specific type is suddenly applied to a resource of a different type. In general we have a functionality $f$ that can be applied to a set of resources $R = \{r_1,r_2,...,r_3\}$ of different type (by type and resource here we do not exclusively mean native types and resources (e.g. files or databases) but more abstract, application specific types (e.g. Eclipse Maven project, Eclipse Java project). This may lead to failure when a functionality that is usually applied to a resource of type $r_1$ is applied to a resource of type $r'$ where $r' \in R \setminus \{r_1\}$.  

\paragraph{\textbf{Scenario}}
\smallskip
This scenario identifies situations where a failure presents when a functionality is applied to a new type of resource.

\paragraph{\textbf{Matching failures}}

\paragraph{Subversive bug report 482565}
\smallskip
%https://bugs.eclipse.org/bugs/show_bug.cgi?id=465574
The failure highlighted by this bug report is that external files in an Eclipse project are marked as obstructed, this means that some functionalities cannot be applied to this type of resource.

\paragraph{EGit bug report 484494}
\smallskip
%https://bugs.eclipse.org/bugs/show_bug.cgi?id=484494
The failure highlighted by this bug report is that when there are symlinks in a project comparing versions with a diff does not show the symlink content on the local side (index side is displayed correctly).

\paragraph{EGit bug report 474019}
\smallskip
%https://bugs.eclipse.org/bugs/show_bug.cgi?id=474019
When cloning a Gerrit repository with http EGit recognizes it correctly and configures it as Gerrit repository, but when it is cloned via SSH it doesn't.

\paragraph{EGit bug report 326526}
\smallskip
%https://bugs.eclipse.org/bugs/show_bug.cgi?id=326526
When pushing commits via ssh with public key authentication EGit asks for password, but even if it is entered correctly it keeps showing the password dialogue without pushing the committed changes.

\paragraph{EGit bug report 474750}
\smallskip
%https://bugs.eclipse.org/bugs/show_bug.cgi?id=474750
\luca{might also be unexpected user input}
When an UTF-8 encoded file is read via the commit viewer they show invalid characters

\paragraph{EGit bug report 435866}
\smallskip
%https://bugs.eclipse.org/bugs/show_bug.cgi?id=435866
EGit asks 3 times for my password and then fails with a TransportException when trying to fetch a repository via https.

\paragraph{\textbf{Test Opportunity}}

\paragraph{Test Trigger}
\smallskip
%Trigger utente crea un istanza di nuovo tipo.
%Installata una nuova funzionalita che fornisce nuovi tipi.
Defining a specific trigger in this case is not trivial: we might identify the triggering action in the user creating or importing a new resource type, or in the application allowing a functionality to be used on different types of resources. 
%l'utente introduce una risorsa di un nuovo tipo -> testo tutte le funzionalità consentite su quel tipo

\subsubsection{Pattern: large resource}

This pattern describes the failures that are triggered by a large resource being handled incorrectly by a functionality of the application under test. An example of incorrectly handling a large resource is trying to load a large database table in memory even if it does not fit, or executing a query on such table and timing out before the results can be generated. In general we have a functionality $f$ that is usually applied to a set of resources $R = \{r_1,r_2,...,r_n\}$, each resource with size $s_i \le s_{safe_i}$; the pattern emerges when a functionality is applied to a resource which has size $s_i > s_{safe_i}$.

\paragraph{\textbf{Scenario}}
\smallskip
This scenario identifies situations where a failure presents when a functionality is handling a large resource in a wrong way.

\paragraph{\textbf{Matching failures}}

\paragraph{Subversive bug report 472752}
\smallskip
%https://bugs.eclipse.org/bugs/show_bug.cgi?id=472752
The situation described by the user is of large projects in the same workspace blocking the save operation of eclipse. When the user tries to save a file a message box is presented to him with the message "wait for user operation to complete". This is due to subversion updating the svn cache and was fixed by moving out long running code from the event listener using queue/asynchronous processing.

\subsection{Obligation: functionality/service coverage}

This obligation is similar to the previous one, but instead of changes in resources we are now interested in changes in services. By services we mean everything that is used by functionalities of the application under test via API. We are interested in testing our application when a service changes (e.g. it is updated to a new version). 

\subsubsection{Pattern: service update}

\luca{generalize}
This pattern presents when a service used by the application is updated. In general we have a service $s$ used by some functionalities $F_s = \{f_1,f_2,...,f_n\}$ of our application; when this service is update to a new version $s'$ it might trigger a failure when the functionalities in $F_s$ are used. 

\paragraph{\textbf{Scenario}}
\smallskip
This scenario identifies situations where a failure is preceded by an update of a service used by the faulty functionality that triggers the failure. This happens when an external service that the functionality uses via API is updated. The failure is typically triggered when the service's API are called by the faulty functionality.

\paragraph{\textbf{Matching failures}}

\paragraph{Subversive bug report 429992}
\smallskip
%https://bugs.eclipse.org/bugs/show_bug.cgi?id=429992
Here a fault is introduced when Java is updated to version 1.8, which introduces lambda expressions, this makes the EclipseLink plugin silently ignore the classes that contain such expressions. \luca{Can a Java update be considered as a service update?}

\paragraph{Subversive bug report 467743}
\smallskip
%https://bugs.eclipse.org/bugs/show_bug.cgi?id=467743
Here a fault is introduced when Eclipse is updated to version 4.4.2 from 4.3, which introduces lambda expressions, this makes the EclipseLink plugin crash with an IncompatibleClassChangeError. \luca{Same as before, this fits the update part of the pattern, but this is not really a service.}

\subsubsection{Pattern: new plugin installed}

This pattern presents when a new plugin is installed in the application framework. In general we have a new plugin $p$ which uses some functionalities $F_p = \{f_1,f_2,...,f_n\}$ of our application (we can see these functionalities as services); when this plugin is installed we are interested in making sure that all of the functionalities in $F$ are working properly. 

\paragraph{\textbf{Scenario}}
\smallskip
This scenario identifies situations where a failure is triggered by a plugin using a faulty functionality of our application.

\paragraph{\textbf{Matching failures}}

\subsection{Obligation: functionality/user input coverage}

This obligation involves covering functionalities of our application that ask for user input. This includes forms that must be filled by the user, command line arguments, GUI buttons, etc.

\subsubsection{Pattern: out-of-domain input value}
\luca{unexpected input value instead of this? e.g. non latin characters}
This pattern presents when the user inputs an out-of-domain value for a specific functionality. This happens for example when non alphanumeric characters are entered a "name" form field, when the same button is clicked multiple times, when invalid command line arguments are entered. Out-of-domain inputs are interesting since these are the cases in which the application failures related to user input are most likely to manifest.

In general we have a functionality $f$ that accepts a set of user inputs $I_f = \{i_1,i_2,...,i_n\}$, we also have a set of input domains $S_d = \{D_1,D_2,..,D_n\}$. This pattern presents when we observe $\exists i_i \in I_f \mid i_i \notin D_i$

\paragraph{\textbf{Scenario}}
\smallskip
This scenario identifies situations where a failure is preceded by an out-of-domain user input. The failure is typically triggered by the application functionality not checking the user input correctly.

\paragraph{\textbf{Matching failures}}

\paragraph{Subversive bug report 459010}
\smallskip
%https://bugs.eclipse.org/bugs/show_bug.cgi?id=459010
This fault presents whenever a user tries to open a folder with a blank space at the end with the subversive UI: svn issues a repository folder children operation failed. \luca{Can we consider a blank in a folder name an out of domain value?}

\paragraph{Subversive bug report 460253}
\smallskip
%https://bugs.eclipse.org/bugs/show_bug.cgi?id=460253
Here the unmarshalling method for a JSON object that has a null attribute incorrectly returns a null value. \luca{A JSON object with an unsetted attribute might not be considered out-of-domain.}

\subsubsection{Pattern: new input sequence}
\luca{in practice this is only feasible if the sequence model is coarse grained}

This pattern presents when the user inputs a new sequence of actions (through clicks in menus for example), in this case new sequence means that such sequence was not previously tested in-house. This type of user behaviour is worth testing because it may lead the testing framework to discover faults that due to their combinatorial nature were not discovered during in-house testing.

In general we have a functionality $f$ that accepts as input a set of sets of user actions $S = \{A_1,A_2,...,A_n\}$ where $A_i = \{a_1,a_2,...,a_n\}$. We are also interested in the set of sets of actions already tested in-house $S_{\texttt{inHouse}}$.  Sequences that are different from the ones tested in-house are not always easy to discover. The trivial case presents when we have a new sequence longer than every previously tested one ($\exists A_i \in S \mid |A_i| > |\texttt{max}\{S_{\texttt{inHouse}}\}|$) but we can also observe a new sequence when it is equal to the ones already tested except for one (or more) elements, without being necessarily longer or shorter.

\paragraph{\textbf{Scenario}}
\smallskip
This scenario identifies situations where a failure is preceded by a new sequence of user actions. The failure is typically triggered by the application being in an incorrect state when the last user action is executed.

\paragraph{\textbf{Matching failures}}

\paragraph{Subversive bug report 470990}
\smallskip
%https://bugs.eclipse.org/bugs/show_bug.cgi?id=470990
Here a broken menu entry is reported by a user who navigated to Preferences / Team / SVN / Label Decorations in the eclipse menu, this entry was probably overlooked by developers and hence constitutes a new input sequence. \luca{bad testing?}

\paragraph{\textbf{Test Opportunity}}

\paragraph{Test Trigger}
\smallskip
The trigger to out testing framework is a user input sequence recognized as new.

\paragraph{Test Strategy}
\smallskip
When we encounter a sequence of actions that was not previously tested we are interested in making sure that the application state is consistent and that other actions executed in that state do not cause the system to crash. In general when a sequence of user actions brings the application in a state $s$ we have a set of actions $A = \{a_1,a_2,...,a_n\}$ that are available in that state; we want to execute each one of these actions and observe the application behaviour.


\subsubsection{Pattern: large input size}

This pattern presents when we have a large user input that was not previously observed or tested.
In general we have a functionality $f$ that accepts a set of user inputs $i$ with max size $s_{\texttt{max}}$ and safe size $s_{\texttt{safe}}$, where $s_{\texttt{safe}}$ was previously observed and tested. This pattern presents when we observe a user input with size between $s_{\texttt{safe}}$ and $s_{\texttt{max}}$.
